Revisiting consistency for semi-supervised semantic segmentation

Semi-supervised learning an attractive technique in practical deployments of deep models since it relaxes the dependence on labeled data. It is especially important in the scope of dense prediction because pixel-level annotation requires significant effort. This paper considers semi-supervised algorithms that enforce consistent predictions over perturbed unlabeled inputs. We study the advantages of perturbing only one of the two model instances and preventing the backward pass through the unperturbed instance. We also propose a competitive perturbation model as a composition of geometric warp and photometric jittering. We experiment with efficient models due to their importance for real-time and low-power applications. Our experiments show clear advantages of (1) one-way consistency, (2) perturbing only the student branch, and (3) strong photometric and geometric perturbations. Our perturbation model outperforms recent work and most of the contribution comes from photometric component. Experiments with additional data from the large coarsely annotated subset of Cityscapes suggest that semi-supervised training can outperform supervised training with the coarse labels.

==> graphical_abstract.tex <==
%\usepackage{newpxtext,newpxmath,scalefnt,cmbright,palatino}
%\renewcommand{\vec}[1]{\bm{#1}}
%\renewcommand*{\familydefault}{\sfdefault}

\usetikzlibrary{fit,automata,arrows,positioning,calc,petri,topaths,arrows.meta,patterns.meta}
\tikzstyle{nrect} = [rectangle, thick, minimum size=8.5mm, draw=black, fill=white, node distance=5mm, rounded corners=0.1ex]
\tikzstyle{circ} = [circle,radius=0.6mm,draw=black,line width=0.3mm,fill opacity=0,inner sep=0.6mm, outer sep=0]
\tikzstyle{textbox} = [text width=10cm,align=left,fill=white!95!themeblue, inner sep=2.5mm, outer sep=0, below right, text ragged]
\tikzstyle{densely dashed}=          [dash pattern=on 2pt off 1.5pt]
\definecolor{themeblue}{RGB}{25,71,163}
\definecolor{arrowcs}{HTML}{cc6611}
\definecolor{arrowct}{HTML}{2288dd}
%\definecolor{arrowct}{HTML}{22aa22}
\tikzset{
    every node/.style={
        outer sep=0
    },
}

\tikzset{
>={Triangle[length=2.4mm,width=2.0mm]},
dedge/.style={arrows=->, black, thick},
}
%\tikzset{
%	double arrow/.style args={#1 in #2 and #3}{
%	-{Stealth[length=(#1)*5, width=4*(#1)]},line width=#1,#2, % first arrow
%	postaction={draw,-{Stealth[length=(#1)*(4-1/4), width=(#1)*(3-1/4)]},#3,line width=(#1)/2,shorten <=(#1)/4,shorten >=2*(#1)/4}, % second arrow
%	}
%}



\scalefont{1.0}

\begin{tikzpicture}[scale=2]

% Background
\fill[fill=themeblue!15!white] (0,0) rectangle (10.5,9.25) node[pos=.5] {};


% Title
\draw (0,9.125) node[text width=19cm, align=left, inner sep=5mm,below right] {
	\scalefont{1.5}{Revisiting Consistency for Semi-Supervised Semantic Segmentation}};


% Consistency variants

\draw (0.25,8.375) node[textbox, text width=8.25cm] (par-variants) {
	We study an extensive set of consistency formulations and find out that \textcolor{arrowct}{one-way consistency with clean teacher} consistently outperforms the others.
	};


\node (sup) [rectangle, fill=white!95!themeblue, inner sep=1.25mm, below left=6mm and -42.5mm of par-variants] {
	\scalebox{-1}[1]{\includegraphics[width=4cm]{figs/semi_toy/semi_toy_kl_detach_clean_detach_pert_20000_2.pdf}}};
\node (sup-text) [fill=white, fill opacity=0.8, text opacity=1, below=-5.5mm of sup] {only supervised};

\node (1wcs) [rectangle, fill=arrowcs, inner sep=1.25mm, right=2.5mm of sup] {
	\scalebox{-1}[1]{\includegraphics[width=4cm]{figs/semi_toy/semi_toy_kl_detach_pert_20000_2.pdf}}};
\node (1wcs-text) [fill=white, fill opacity=0.8, text opacity=1, below=-5.5mm of 1wcs] {one-way, clean student};

\node (1wct) [rectangle, fill=arrowct, inner sep=1.25mm, below=2.5mm of sup] {
	\scalebox{-1}[1]{\includegraphics[width=4cm]{figs/semi_toy/semi_toy_kl_detach_clean_20000_2.pdf}}};
\node (1wct-text) [fill=white, fill opacity=0.8, text opacity=1, below=-5.5mm of 1wct] {one-way, clean teacher};

\node (2wc1) [rectangle, fill=arrowct, inner sep=1.25mm, below=2.5mm of 1wcs, postaction={pattern={Lines[angle=-45, distance=5mm, line width=2.5mm]}}, pattern color=arrowcs] {
	\scalebox{-1}[1]{\includegraphics[width=4cm]{figs/semi_toy/semi_toy_kl_20000_2.pdf}}};
\node (2wc1-text) [fill=white, fill opacity=0.8, text opacity=1, below=-5.5mm of 2wc1] {two-way, one input clean};

\draw node[circ, below right=-14.5mm and -15.23 mm of 1wcs,opacity=0.5] (clean1wcs) {};
\draw node[circ, below right=-14.5mm and -15.23 mm of 1wct,opacity=0.5] (clean1wct) {};
\draw node[circ, below right=-14.5mm and -15.23 mm of 2wc1,opacity=0.5] (clean2wc1) {};
\draw node[circ, below right=-15mm and -9 mm of 1wcs] (pert1wcs) {};
\draw node[circ, below right=-15mm and -9 mm of 1wct] (pert1wct) {};
\draw node[circ, below right=-15mm and -9 mm of 2wc1] (pert2wc1) {};
\path (pert1wcs) edge [dedge,-{Triangle[length=5*0.4mm, width=4*0.4mm]}] node (1wcs-edge) {} (clean1wcs);
\path (clean1wct) edge [dedge,-{Triangle[length=5*0.4mm, width=4*0.4mm]}] node (1wct-edge) {} (pert1wct);
\path (clean2wc1) edge [dedge,-{Triangle[length=5*0.4mm, width=4*0.4mm]}] node (2wc1-edge) {} (pert2wc1);
\path (pert2wc1) edge [dedge,-{Triangle[length=5*0.4mm, width=4*0.4mm]}] node {} (clean2wc1);

%labels: unlabeled, labeled, perturbed
{\scalefont{0.8}
\node (labeled-text) [fill=white, fill opacity=0.8, text opacity=1, below right=-12mm and -14 mm of sup] {labeled examples};
%\draw node[circ, below right=-12.95mm and -17.05 mm of sup,opacity=0.5] (labeled1) {};
\draw node[circ, below right=-21.25mm and -7.65 mm of sup,opacity=0.5] (labeled2) {};
\draw node[circ, below right=-10.6mm and -31.2 mm of 1wcs,opacity=0.5] (labeled3) {};
%\path (labeled-text) edge [-stealth, thick, densely dashed] node {} (labeled1);
\path (labeled-text) edge [-stealth, thick, densely dashed] node {} (labeled2);
\path (labeled-text) edge [-stealth, thick, densely dashed] node {} (labeled3);

\node (unlabeled-text) [fill=white, fill opacity=0.8, text opacity=1, below right=-29mm and -4mm of sup] {unlabeled examples};
\draw node[circ, below right=-27.3mm and -10.1 mm of sup,opacity=0.5] (unlabeled1) {};
\draw node[circ, below right=-18.48mm and -35.55 mm of 1wcs,opacity=0.5] (unlabeled3) {};
\path (unlabeled-text) edge [-stealth, thick, densely dashed] node {} (unlabeled1);
\path (unlabeled-text) edge [-stealth, thick, densely dashed] node {} (unlabeled3);

\node (clean-text) [fill=white, fill opacity=0.8, text opacity=1, below right=-16.2mm and -28 mm of 2wc1] {clean};
\path (clean-text) edge [-stealth, thick, densely dashed] node {} (clean2wc1);

\node (perturbed-text) [fill=white, fill opacity=0.8, text opacity=1, below right=-11mm and -16 mm of 2wc1] {perturbed};
\path (perturbed-text) edge [-stealth, thick, densely dashed] node {} (pert2wc1);

\node (direction-text) [fill=white, fill opacity=0.8, text opacity=1, below right=-31mm and -4mm of 1wct, text width=2.63cm] {consistency direction (teacher to student)};
\path (direction-text) edge [-stealth, thick, densely dashed] node {} (1wct-edge);
\path (direction-text) edge [-stealth, thick, densely dashed] node {} (2wc1-edge);
}


% Risky-useful illustration

\node (par-inputs) [textbox, text width=8.25cm, below=79.5mm of par-variants] {
	Predictions in \textcolor{arrowct}{clean inputs} are better consistency targets due to being more often correct than predictions in \textcolor{arrowcs}{perturbed inputs}.
	%Predictions in \textcolor{arrowcs}{perturbed inputs} are poor consistency targets due to being more often incorrect.
	};

\draw node[rectangle, fill=arrowct, inner sep=1.25mm, below left=6mm and -42.5mm of par-inputs] (xu) {
	\includegraphics[width=4cm]{figs/training/38_x_u.png}};
\draw node[opacity=0.5, right=-4.25cm of xu] (outu) {
	\includegraphics[width=4cm]{figs/training/38_out_u.png}};
\draw node[rectangle, fill=arrowcs, inner sep=1.25mm, right=2.5mm of xu] (xp) {
	\includegraphics[width=4cm]{figs/training/38_x_p.png}};
\draw node[opacity=0.5,right=-4.25cm of xp] (outp) {
	\includegraphics[width=4cm]{figs/training/38_out_p.png}};

\draw node[circ, below right=-35.1mm and -11.5 mm of xu] (Ac) {};
\draw node[circ, below right=-36.2mm and -5.7 mm of xp] (Ap) {};
%\draw [double arrow=1.2mm in black and arrowcs] (Ap) to [in=15,out=165] (Ac);
\draw[arrowcs,line width=1mm,-{Triangle[length=5*0.8mm, width=4*0.8mm]}] (Ap) to [in=15,out=165] (Ac);

\draw node[circ, below right=-25mm and -28mm of xu] (Bc) {};
\draw node[circ, below right=-19mm and -24.4mm of xp] (Bp) {};
%\draw [double arrow=1.2mm in black and arrowct] (Bc) to [out=-25,in=185] (Bp);
\draw[arrowct,line width=1mm,-{Triangle[length=5*0.8mm, width=4*0.8mm]}] (Bc) to [out=-25,in=185] (Bp);

\draw node[fill=white, text opacity=1, fill opacity=0.8, align=center,inner sep=0.5mm, below right=-35mm and -45mm of xp] (cs) {
	clean student and};
\node[fill=white, text opacity=1, fill opacity=0.8, align=center,inner sep=0.5mm,below=0 of cs] {
	perturbed teacher: risky};
\draw node[fill=white, text opacity=1, fill opacity=0.8, align=center,inner sep=0.5mm, below right=-14mm and -22mm of xu] (ct) {
	clean teacher and};
\node[fill=white, text opacity=1, fill opacity=0.8, align=center,inner sep=0.5mm,below=0 of ct] {
	perturbed student: useful};
%\draw (3.3,3.5) node[fill=white, text opacity=1, fill opacity=0.8, align=center,below=0 of outu] (cs) {
%	clean};
%\draw (3.3,3.5) node[fill=white, text opacity=1, fill opacity=0.8, align=center,below=0 of outp] (cs) {
%	perturbed};


% Consistency loss computational graph

\draw (6.5,4) node[nrect] (x) [] {$\vec x$};

\draw (7.5,4.5) node[nrect] (y) [] {$h_{\vec\theta'}$};
\draw (8.5,4.5) node[nrect] (tp) [] {$T^\text{G}_{\vec\gamma}$};
\draw (7.5,3.5) node[nrect] (xp) [] {$T^\text{G}_{\vec\gamma}\circ T^\text{P}_{\vec\varphi}$};
\draw (8.5,3.5) node[nrect, themeblue, fill=white!95!themeblue] (yp) [] {$h_{\vec\theta}$};
\draw (9.5,4) node[nrect, themeblue, fill=white!95!themeblue] (D) [] {$D$};
%\node[above=0 of y] {$\vec y$};
%\node[below=0 of tp] {$\vec y$};

\node (imx) [left=0 of x] {
	\includegraphics[width=1.5cm]{figs/training/38_x_u.png}};
\node (imy) [above=0 of y] {
	\includegraphics[width=1.5cm]{figs/training/38_out_u.png}};
\node (imtp) [above=0 of tp] {
	\includegraphics[width=1.5cm]{figs/training/38_out_t.png}};
\node (imxp) [below=0 of xp] {
	\includegraphics[width=1.5cm]{figs/training/38_x_p.png}};
\node (imyp) [below=0 of yp] {
	\includegraphics[width=1.5cm]{figs/training/38_out_p.png}};

\path (x) edge [dedge] node {} (y);
\path (y) edge [dedge] node {} (tp);
\path (x) edge [dedge] node {} (xp);
\path (xp) edge [dedge] node {} (yp);
\path (tp) edge [dedge, style={arrows=->||}] node {} (D);
\path (yp) edge [dedge, themeblue] node {} (D);

{\scalefont{0.8}
%\node (input) [below=0 of x] {input};
\node (teacher) [fill=white, fill opacity=0.8, text opacity=1, above left=-5mm and 4mm of y] {teacher};
\path (teacher) edge [-stealth, thick, densely dashed] node {} (y);
\node (student) [fill=white, fill opacity=0.8, text opacity=1, above=3mm of yp] {student};
%\node (grad) [fill=white, fill opacity=0.8, text opacity=1, below right=1.25mm of yp, text width=2cm, text badly ragged] {gradient computed only here};
\path (student) edge [-stealth, thick, densely dashed] node {} (yp);
\node (pert)    [fill=white, fill opacity=0.8, text opacity=1, below left=-2.5mm and 4mm of xp] {perturbation};
\path (pert) edge [-stealth, thick, densely dashed] node {} (xp);
\node (outpert) [fill=white, fill opacity=0.8, text opacity=1, above right=-7.5mm and 4mm of tp, text ragged, align=left] {perturbation\\(equivariance)};
\path (outpert) edge [-stealth, thick, densely dashed] node {} (tp);
\node (diverg)  [fill=white, fill opacity=0.8, text opacity=1, below=3mm of D] {divergence};
\path (diverg) edge [-stealth, thick, densely dashed] node {} (D);
}

\draw (5,8.375) node[textbox] (par-oneway) {
	One-way consistency is especially convenient in the dense prediction context due to entailing the same memory footprint as in the supervised case.
	};
	
\draw node[textbox, below=5mm of par-oneway] (par-graph)  {
	Our composite perturbations allow to learn from photometric ($T^\text{P}_{\vec\varphi}$) invariance and geometric ($T^\text{G}_{\vec\gamma}$) equivariance.
	Photometric perturbations contribute more on Cityscapes.
	\\\vspace{2.5mm}
	The teacher parameters $\vec\theta'$ are a frozen copy of the student parameters $\vec\theta$; they do not contribute to the gradients.
	};

\draw node[textbox, below=71.5mm of par-graph] {Contributions:
	\begin{itemize}
		\setlength\itemsep{0mm}
		\item explanation of advantages of one-way consistency with clean teacher,
		\item novel perturbation model that allows concurrent learning from photometric invariance and geometric equivariance,
		\item empirical evaluation on efficient models under small and large data regimes.
	\end{itemize}};

\end{tikzpicture}

